Improved Neural Text Attribute Transfer with Non-parallel Data

Text attribute transfer using non-parallel data requires methods that can perform disentanglement of content and linguistic attributes. In this work, we propose multiple improvements over the existing approaches that enable the encoder-decoder framework to cope with the text attribute transfer from non-parallel data. We perform experiments on the sentiment transfer task using two datasets. For both datasets, our proposed method outperforms a strong baseline in two of the three employed evaluation metrics.

==> acknowledgements.tex <==
%\subsubsection*{Acknowledgments}

%Use unnumbered third level headings for the acknowledgments. All
%acknowledgments go at the end of the paper. Do not include
%acknowledgments in the anonymized submission, only in the final paper.


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The ideas proposed in this paper are  original and open a different direction in the use of adversarial networks (AD). To the best of our knowledge, so far, adversarial networks have been used only in setups that include a generator, and almost all works on AD use computer vision tasks in their experiments.
We have not found any paper on using adversarial networks to learn the loss function of predictors.
Our experimental results demonstrate that for both tasks DAN consistently boosts the predictor's performance when only few labeled instances are available.
Moreover,
in terms of learning accurate predictors, the loss functions automatically learned by DAN are as effective as the loss functions commonly used for text ranking and classification.

In our experiments we have used simple architectures in both predictor and judge in order to make it easier to check the real contribution of the proposed approach.
Although our architectures for both \emph{predictors} are not new, the judge architectures contain some novelties, such as the scoring function used in the classification task. We have also experimented using a judge that performs classification by concatenating the representation of the sentence ($r_s$) with the (soft) representation of the predicted $\hat{y}$ ($r_{pos}$), and then use the resulting vector to perform logistic regression. 
However,
the training is unstable and the DAN cannot learn.

The main drawback of using ADs is that the min-max game makes the training a bit more challanging.
We believe that part of the instability in the results for SSL (sometimes CNN-DAN$_{unlab.}$ is worse than CNN-DAN) is due to the difficulties of properly training the DAN.
We have tried some tricks used for training GANs such as minibatch discrimination and feature matching \cite{salimans2016improved}, and have also tried WGAN \cite{arjovsky17a}, but none of these alternatives helped much for our two architectures.
In future work, we would like to try the ideas from FisherGAN \cite{mrouehS17fishergan} and ImprovedWGAN \cite{GulrajaniImprovedWGAN17} which have demonstrated good results on stabilizing the training of GANs.

Structured prediction problems that normally use surrogate (not optimal) loss functions can benefit from DAN's implicit loss function learning capability. 
On the other hand, the aplication of DANs for some structured prediction tasks can be challenging because the output of the predictor needs to be continuous since we need to backpropagate through it.  
However,
this is not a big problem because most NLP tasks with structured outputs are solved using predictors that produce continuous outputs over elements of the structure.
For instance,
in ranking, 
normally the output is a (continuous) ranking score for each document; and
in the case of coreference resolution,
usually the predictor outputs a score for each pair of mentions in the input document.
